Privacy-Preserving Set-Based Estimation Using Differential Privacy and Zonotopes

For large-scale cyber-physical systems, the collaboration of spatially distributed sensors is often needed to perform the state estimation process. Privacy concerns arise from disclosing sensitive measurements to a cloud estimator. To solve this issue, we propose a differentially private set-based estimation protocol that guarantees true state containment in the estimated set and differential privacy for the sensitive measurements throughout the set-based state estimation process within the central and local differential privacy models. Zonotopes are employed in the proposed differentially private set-based estimator, offering computational advantages in set operations. We consider a plant of a non-linear discrete-time dynamical system with bounded modeling uncertainties, sensors that provide sensitive measurements with bounded measurement uncertainties, and a cloud estimator that predicts the system's state. The privacy-preserving noise perturbs the centers of measurement zonotopes, thereby concealing the precise position of these zonotopes, i.e., ensuring privacy preservation for the sets containing sensitive measurements. Compared to existing research, our approach achieves less privacy loss and utility loss through the central and local differential privacy models by leveraging a numerically optimized truncated noise distribution. The proposed estimator is perturbed by weaker noise than the analytical approaches in the literature to guarantee the same level of privacy, therefore improving the estimation utility. Numerical and comparison experiments with truncated Laplace noise are presented to support our approach.

==> Sections/extras.tex <==
%extras abstract
\st{upholds the privacy of sets containing sensitive measurements} 






To illustrate the practical relevance of the problem statement, consider the following scenario:
\begin{example}
% A cloud estimator of an ITS can use locations and routing data, voluntarily shared by Autonomous vehicles, to provide safe paths through intersections and zebra crossings for pedestrians and scooter drivers. Autonomous vehicles are connected to each other and to the infrastructure of the ITS. These vehicles send measurement sets to a cloud estimator. The cloud estimator in turn uses these measurement sets received from autonomous vehicles and the data collected from sensors, cameras, GPS, and cell phones to manage smart traffic lights and detect patterns of traffic, to provide safe paths through intersections and zebra crossings for pedestrians and scooter drivers. 

A cloud estimator in an ITS can utilize location and routing data, voluntarily shared by autonomous vehicles, to ensure safe paths through intersections and zebra crossings for pedestrians and scooter drivers. These autonomous vehicles are interconnected and linked to the ITS infrastructure, sending measurement sets to the cloud estimator. The cloud estimator uses these measurement sets, along with data collected from sensors, cameras, GPS, and cell phones, to manage smart traffic lights and detect traffic patterns, thereby enhancing safety at intersections and zebra crossings.
\end{example}







\begin{align}
	% \Acute{c}^{DP}_k = & \hat{c}^{DP}_{k} + \sum_{i=1}^{m} \lambda^{(i)}_{k} \big ( \hat{y}^{(i)^{DP}}_{k} -  h^{(i)}(x_{k}^{*}) - c^{(i)}_{v}-c_{p} \big) \\
 \Acute{c}^{DP}_k =&  \hat{c}^{DP}_{k} + \sum_{i=1}^{m} \lambda^{(i)}_{k} \bigg( y^{(i)^{DP}}_{k} - h^{(i)}\big({x_{k}^{*(i)}}\big)\nonumber\\ 
&-\frac{\partial h_{k}^{(i)}}{\partial x}|_{x_{k}^{*(i)}}(\hat{c}^{DP}_{k} {-} x^{*(i)}_{k}) {-} c^{(i)}_{L,k} 
% -c_{p} - c^{(i)}_{v} 
\bigg),\label{eqn:dp-estimation-with-zonotope-center-non-linear}\\
   % \nonumber \Acute{G}^{DP}_k{=} &\Big[(I- \sum_{i=1}^{m+1} \lambda^{(i)}_{k} \frac{\partial h_{k}^{(i)}}{\partial x}|_{x_{k}^{*}})\hat{G}^{DP}_{k},\\& \lambda^{(1)}_{k}G^{(1)}_{v},\dots, \lambda^{(m)}_{k}G^{(m)}_{v},\lambda^{(m+1)}_{k}G_{p}  \Big],\\
   \Acute{G}^{DP}_k =&\bigg[\bigg(I- \sum_{i=1}^{m} \lambda^{(i)}_{k} 
    \frac{\partial h_{k}^{(i)}}{\partial x}|_{x_{k}^{*(i)}}
    \bigg) \hat{G}^{DP}_{k},\;-\lambda^{(1)}_{k} G^{(1)}_{L,k},\dots, \;\nonumber\\& -\lambda^{(m)}_{k} G^{(m)}_{L,k},-\lambda^{(1)}_{k}G_{p},\dots,-\lambda^{(m)}_{k}G_{p},\;\nonumber\\& -\lambda^{(1)}_{k}G^{(1)}_{v}, \dots, -\lambda^{(m)}_{k}G^{(m)}_{v}  \bigg],\label{eqn:dp-estimation-with-zonotope-generator-non-linear}
\end{align}
where $\mathcal{\Bar{Z}}^{DP}_k=\zono{\Bar{c}^{DP}_k, \Bar{G}^{DP}_k}$ is the corrected state set that is obtained by the reduction of $\mathcal{\Acute{Z}}^{DP}_{k}=\zono{\Acute{c}^{DP}_{k}, \Acute{G}^{DP}_{k}}$, $\mathcal{\hat{Z}}^{DP}_{k}=\zono{\hat{c}^{DP}_{k}, \hat{G}^{DP}_{k}}$ is the predicted state set, $x_{k}^{*(i)}$ is the linearization point for sensor $i$ at time step $k$, 
%\st{${M}_y:\hat{y}^{DP}_k = y_k + \Phi_k$,} 
% $c_{p}$ is the noise value at the center of the truncated optimal noise distribution,
and $G_{p}$ is the generator matrix, created using the range of the optimal noise $d$.












Likewise in \eqref{eqn:estimation-with-zonotope-generator-non-linear}, $\lambda^{(i)}_{k}\in \mathbb{R}^{n\times 1}$ are weights such that $ i \in \{1,\dots,\; m\}$. Again, as in \cite{conf:disdiff}, the optimal weights $\lambda^{(i)}_{k}$ are calculated by 
\begin{equation}\label{eqn:dp-optimal-lambda-weights}
\Bar{\Lambda}_k^* = \argminB_{{\lambda}_k}\lVert \Acute{G}^{DP}_k \rVert_{F}^{2},
\end{equation}
where $\Bar{\Lambda}_k^* = [ {\lambda}^{(1)}_{k},\dots,\; {\lambda}^{(m)}_{k}]$. 
Next, the order of generator matrix $\Acute{G}^{DP}_k$ is reduced according to \cite{10.1007/978-3-540-31954-2_19}, 
then we get $\mathcal{\Bar{Z}}^{DP}_k=\zono{\Bar{c}^{DP}_k,\Bar{G}^{DP}_k}$.

The prediction update according to the system model defined in \eqref{eqn:system-model-non-linear}, is given by
\begin{equation}\label{eqn:dp-time-update}
    \mathcal{\hat{Z}}^{DP}_{k}=f(\mathcal{\Bar{Z}}^{DP}_{k-1})\oplus \mathcal{Z}_w,
\end{equation}
where $\mathcal{\hat{Z}}^{DP}_k=\zono{\hat{c}^{DP}_k, \hat{G}^{DP}_k}$ is the predicted state set. 
% represented by the zonotope 
% $\mathcal{\hat{Z}}^{DP}_k=\zono{\hat{c}^{DP}_k, \hat{G}^{DP}_k}$.

Finally, we summarize the differentially private set-based estimator in Algorithm \ref{alg:adp-set-estimation-using-zonotope}. 


%estimator extras

\begin{enumerate}[leftmargin=*]
\item {Prediction step:} Consider the past corrected state set $\mathcal{\Bar{Z}}_{k-1}$ and a process noise $w_k \in \mathcal{Z}_w$. The set-based state estimator determines the predicted state set $\mathcal{\hat{Z}}_{k}$, which is a set of all reachable states, computed as
\begin{align}\label{eqn:predicted-state-set}
	\mathcal{\hat{Z}}_{k}  = f(\mathcal{\Bar{Z}}_{k-1})\oplus \mathcal{Z}_w.
\end{align}
\item {Correction step:} The corrected state set $\mathcal{\Bar{Z}}_{k}$ is determined using the predicted state set $\mathcal{\hat{Z}}_{k}$ \eqref{eqn:predicted-state-set}, the measurement sets corresponding to $\{y^{(i)}_k \}_{k\in\mathbb{Z^+}}$, and some weights $\lambda^{(i)}_{k}$, $i \in \{1,\dots,m\}$ according to the following lemma.
\end{enumerate}


%lemma1 extras



\begin{lemma}[\cite{9838494,9811706}] \label{lemma-set-based-estimation-zonotope-non-linear} 
The intersection between the predicted state set $\mathcal{\hat{Z}}_{k}=\zono{\hat{c}_{k}, \hat{G}_{k}}$ and the $m$ measurement sets $\mathcal{Z}^{(i)}_{y_k}$ is over-approximated by $\mathcal{\Acute{Z}}_k = \zono{\Acute{c}_k, \Acute{G}_k}$
 
% Let $x_0 \in \mathcal{\Bar{Z}}_0{=}\zono{\Bar{c}_0,\Bar{G}_0}$ and $v^{(i)}_{k} \in \mathcal{Z}^{(i)}_{v}{=}\zono{0,G^{(i)}_{v}}$. Then,


% the corrected state set $\mathcal{\Bar{Z}}_{k}$ is computed using a zonotope $\mathcal{\Acute{Z}}_k=\zono{\Acute{c}_k, \Acute{G}_k}$ over-approximating the intersection between 
% the zonotope $\mathcal{\hat{Z}}_{k}=\zono{\hat{c}_{k}, \hat{G}_{k}}$ representing 
% the predicted state set $\mathcal{\hat{Z}}_{k}=\zono{\hat{c}_{k}, \hat{G}_{k}}$ and the $m$ regions for $x_k$ states corresponding to $y^{(i)}_{k}$, where

% \begin{align}
% 	\Acute{c}_k &=  \hat{c}_{k} + \sum_{i=1}^{m} \lambda^{(i)}_{k} \big ( y^{(i)}_{k} - H^{(i)} \hat{c}_{k} - c^{(i)}_{v} \big), \label{eqn:estimation-with-zonotope-center}\\
%     \Acute{G}_k &=\big[(I- \sum_{i=1}^{m} \lambda^{(i)}_{k} H^{(i)})\hat{G}_{k}, \; \lambda^{(1)}_{k}G^{(1)}_{v}, \dots, \lambda^{(m)}_{k}G^{(m)}_{v} \big],\label{eqn:estimation-with-zonotope-generator}
% \end{align}
% where $\mathcal{\Acute{Z}}_{k}=\mathcal{\Acute{Z}}_{k}=\zono{\Acute{c}_{k}, \Acute{G}_{k}}$, and $\lambda^{(i)}_{k}\in \mathbb{R}^{n\times 1}$ are weights such that $ i \in \{1,\dots,\; m\}$ and $k\in \mathbb{Z}^+$.
\end{lemma}
\begin{proof}
The proof follows directly from \cite[Proposition 2]{9838494} and \cite[Theorem 1]{9811706}.
\end{proof}


, as follows: 
\begin{align}\label{eqn:optimal-lambda-weights}
\Bar{\Lambda}_k = \argminB_{\lambda_k} \, \lVert \Acute{G}_k \rVert_{F}^{2}.
\end{align}

 are computed

\begin{align}
	\Acute{c}_k= &  \hat{c}_{k} + \sum_{i=1}^{m} \lambda^{(i)}_{k} \bigg ( y^{(i)}_{k} - h^{(i)}\big({x_{k}^{*(i)}}\big)\nonumber\\ 
&-\frac{\partial h_{k}^{(i)}}{\partial x}|_{x_{k}^{*(i)}}\big(\hat{c}_{k} {-} x^{*(i)}_{k}\big) {-} c^{(i)}_{L,k} \bigg), \label{eqn:estimation-with-zonotope-center-non-linear}\\
    \Acute{G}_k =&\bigg[\bigg(I- \sum_{i=1}^{m} \lambda^{(i)}_{k} 
    % \mathbb{J}^{(i)}_{h}(\hat{c}_{k}) 
    \frac{\partial h_{k}^{(i)}}{\partial x}|_{x_{k}^{*(i)}}
    \bigg) \hat{G}_{k},-\lambda^{(1)}_{k} G^{(1)}_{L,k},\dots, \;\nonumber\\& -\lambda^{(m)}_{k} G^{(m)}_{L,k},-\lambda^{(1)}_{k}G^{(1)}_{v}, \dots, -\lambda^{(m)}_{k}G^{(m)}_{v}  \bigg],\label{eqn:estimation-with-zonotope-generator-non-linear}
\end{align}
where 
% $\mathcal{\Acute{Z}}_{k}=\zono{\Acute{c}_{k}, \Acute{G}_{k}}$,
$x_{k}^{*(i)}$ is the linearization point for sensor $i$ at time step $k$, and $\lambda^{(i)}_{k}\in \mathbb{R}^{n\times 1}$ are weights such that $ i \in \{1,\dots,\; m\}$ and $k\in \mathbb{Z}^+$.





% algorithm extras
\State 
Obtain a sensitive measurement $y_k^{(i)}$ from each sensor $i$, where $ i\in \{1,\dots,\; m\}$. \label{line:2-start-add-noise}
\If{the CDP model is deployed}
\State The sensor manager aggregates the $m$ measurements into a vector of measurements $y_k=\big[{y_k^{(1)}},\dots,{y_k^{(m)}}\big]^T$. 
{\State The sensor manager adds the privacy-preserving noise to the measurements to obtain protected measurements $\hat{y}^{DP}_k$ following \eqref{eqn:additive-noise-mechanism}.}
\ElsIf{the LDP model is deployed}
\State Each sensor locally perturbs its own measurement to obtain a protected measurement $\hat{y}^{(i)^{DP}}_k$ according to \eqref{eqn:additive-noise-mechanism-ldp-measurement}.
\EndIf \label{line:8-end-add-noise}







{\color{blue}
\begin{equation}\label{eqn:dp-time-update}
    \mathcal{\hat{Z}}^{DP}_{k}=f^{\text{lin}}(\mathcal{\Bar{Z}}^{DP}_{k-1})\oplus \mathcal{Z}_w \oplus \mathcal{\Bar{Z}}_{L,k},
\end{equation}\label{line:10-predicted-state-set} where $f^{\text{lin}}$ is the linearization of the state function $f$ using Taylor series and $\mathcal{\Bar{Z}}_{L,k} = \zono{c_{L,k}, G_{L,k}}$ is its Lagrange remainder.}


using the predicted state set $\mathcal{\hat{Z}}_{k}$ \eqref{eqn:predicted-state-set}, the measurement sets 
% corresponding to $\{y^{(i)}_k \}_{k\in\mathbb{Z^+}}$
$\mathcal{Z}^{(i)}_{y_k}$, and some weights $\lambda^{(i)}_{k}$, $i \in \{1,\dots,m\}$ in lines \ref{line:correction-start-alg-1} to \ref{line:correction-end-alg-1}.
\State\begin{align}
    \Acute{c}_k =&  \hat{c}_{k} + \sum_{i=1}^{m} \lambda^{(i)}_{k} \bigg( y^{(i)}_{k} - h^{(i)}\big({x_{k}^{*(i)}}\big)\nonumber\\ 
&-\frac{\partial h_{k}^{(i)}}{\partial x}|_{x_{k}^{*(i)}}(\hat{c}_{k} {-} x^{*(i)}_{k}) {-} c^{(i)}_{L,k} 
% -c_{p} - c^{(i)}_{v} 
\bigg),\label{eqn:estimation-with-zonotope-center-non-linear}
\end{align}

\label{line:correction-start-alg-1}
\State  
\begin{align}
    \Acute{G}_k =&\bigg[\bigg(I- \sum_{i=1}^{m} \lambda^{(i)}_{k} 
    \frac{\partial h_{k}^{(i)}}{\partial x}|_{x_{k}^{*(i)}} \bigg) \hat{G}_{k},\;-\lambda^{(1)}_{k} G^{(1)}_{L,k},\dots, \;\nonumber\\& -\lambda^{(m)}_{k} G^{(m)}_{L,k}, -\lambda^{(1)}_{k}G^{(1)}_{v}, \dots, -\lambda^{(m)}_{k}G^{(m)}_{v}  \bigg],\label{eqn:estimation-with-zonotope-generator-non-linear}
\end{align} 
where $x_{k}^{*(i)}$ is the linearization point for sensor $i$ at time step $k\in \mathbb{Z}^+$. The infinite Taylor series is over-approximated by the first-order Taylor series and its Lagrange remainder $\mathcal{\Bar{Z}}^{(i)}_{L,k} = \zono{c^{(i)}_{L,k}, G^{(i)}_{L,k}}$ to guarantee true state inclusion.
%where for sensor $i$, $h^{(i)}(x_k)$ is linearized at $x_{k}^{*(i)}$ and the infinite Taylor series is over-approximated by the first order Taylor series and its Lagrange remainder $\mathcal{\Bar{Z}}^{(i)}_{L,k} = \zono{c^{(i)}_{L,k}, G^{(i)}_{L,k}}$ to guarantee the true state inclusion.
\State Compute the weights $\Bar{\Lambda}_k$
\begin{equation}\label{eqn:dp-optimal-lambda-weights}
\Bar{\Lambda}_k = \argminB_{{\lambda}_k}\lVert \Acute{G}_k \rVert_{F}^{2},
\end{equation}
where $\Bar{\Lambda}_k = [ {\lambda}^{(1)}_{k},\dots,\; {\lambda}^{(m)}_{k}]$. \label{line:optimal-weights-alg-1} 
\State Reduce the order of $\Acute{G}_k$ 
as in \cite{10.1007/978-3-540-31954-2_19}: $\Bar{G}_{k} =\downarrow_q	\Acute{G}_k$. 
\State $\Bar{c}_k = \Acute{c}_k$.
\State $\mathcal{\Bar{Z}}_{k}= \zono{\Bar{c}_k, \Bar{G}_k}$. \label{line:correction-end-alg-1}






%%k figure of example
\begin{figure}[H]
\graphicspath{ {./Figures/} }
    \centerline{
\includegraphics
[width=8.4cm, height=4.5cm]{Figures/measurements-z}}
    \caption{A smart city, in which Autonomous vehicles send measurement sets periodically to the cloud estimator, which estimates safe paths through intersections and zebra crossings for pedestrians and scooter drivers.}
    \label{fig:smart-city}
\end{figure}




% extras of preliminaries and setup

{\color{blue}The CDP and LDP models of differential privacy can be described in detail as follows:}

\begin{itemize}
    \item {Central Differential Privacy (CDP):} 
    % The traditional model of differential privacy, in which a trusted data curator adds uncertainty (e.g., random noise) to the results of any processing on a centrally-held dataset to preserve the privacy of the participants in this dataset and prevent any untrusted party from inferring knowledge about an individual participant \cite{10.5555/3310435.3310586}.
    This traditional model of differential privacy involves a trusted data curator adding uncertainty, such as random noise, to the results of any processing on a centrally held dataset. This is done to safeguard the privacy of participants in the dataset and prevent any untrusted party from deducing information about individual participants \cite{10.5555/3310435.3310586}.
    \item {Local Differential Privacy (LDP):} 
    % In this model of differential privacy, the data of each Participant is locally perturbed, and the privacy-preserving process is transferred from the data curator to individual participants
    In this model of differential privacy, instead of centrally perturbing the data, each participant perturbs their own data locally before sharing it. This decentralized approach shifts the responsibility of privacy preservation from a central data curator to individual participants. Each participant adds noise to their own data before transmitting it to the data curator or any other party, ensuring that privacy is preserved at the local level \cite{Xiong2020}. 
\end{itemize}





%k extras of section 3 algorithm
we employ either of the two additive noise mechanisms described in Definitions \ref{def:additive-noise-mechanism-ldp-measurement} and \ref{def:additive-noise-mechanism}, to introduce perturbations to the sensitive measurements. 















\begin{algorithm}
\caption{($\epsilon, \delta$)-ADP Set-Estimation Using Zonotopes}\label{alg:adp-set-estimation-using-zonotope}
\begin{algorithmic} [1]
{\Statex {\bfseries Input:} DP parameter $\epsilon$, noise range $d$, sensitivity{\color{blue}, 
  process noise zonotope $\mathcal{Z}_w= \zono{0, G_w}$, privacy-preserving noise zonotope $\mathcal{Z}_p= \zono{0, G_p}$, where $G_{p}$ is the generator matrix, created using the range of the optimal noise $d$, and 
  measurement noise zonotopes $\mathcal{Z}^{(i)}_{v}= \zono{0, G^{(i)}_{v}}$, where $i \in \{1, \dots, m\}$}.
} 
{ \Statex {\bfseries Output:} $\mathcal{\Bar{Z}}^{DP}_{k}=\zono{\Bar{c}^{DP}_k, \Bar{G}^{DP}_k}$.}
\Statex{\bfseries Initialization:} The sensor manager uses $\epsilon$, $d$, and sensitivity to generate the truncated optimal noise distribution $P(\phi_l)$ according to \eqref{eqn:optimal-noise-function} while optimizing the loss function in \eqref{eqn:optimization-function} by learning the parameters of the noise model in \eqref{eqn:noise-model}. 
Set $k = 1$ and $\mathcal{\Bar{Z}}_{0} = \zono{\Bar{c_0},\Bar{G_0}}$.
\While{$True$}
\State 
% $m$ sensitive measurements $y_k^{(i)}$, $ i\in \{1,\dots,\; m\}$ provided by an array of $m$ sensors.
Obtain a sensitive measurement $y_k^{(i)}$ from each sensor $i$, where $ i\in \{1,\dots,\; m\}$. \label{line:2-start-add-noise}
% An array of $m$ sensors, where each sensor provides a sensitive measurement $y_k^{(i)}$, $ i\in \{1,\dots,\; m\}$.
\If{the setup in Figure \ref{fig:Centralized-DP-Setting} is deployed}
\State The sensor manager aggregates the $m$ measurements into a vector of measurements $y_k=\big[{y_k^{(1)}},\dots,{y_k^{(m)}}\big]^T$. 
{\State The sensor manager adds the DP noise to 
$y_k$ to obtain protected measurements
% uses the additive noise mechanism $M_y$ (Definition \ref{def:additive-noise-mechanism}) to obtain 
$\hat{y}^{DP}_k$ following \eqref{eqn:additive-noise-mechanism}.}
\algstore{myalg-dp}
\end{algorithmic}
\end{algorithm}
\begin{algorithm}
\begin{algorithmic} [1]
\algrestore{myalg-dp}
\ElsIf{the setup in Figure \ref{fig:local-DP-Setting} is deployed}
\State Each sensor locally perturbs its own measurement 
% using the additive noise mechanism ${M}^{(i)}_y$ (Definition \ref{def:additive-noise-mechanism-ldp-measurement}) 
to obtain a protected measurement $\hat{y}^{(i)^{DP}}_k$ according to \eqref{eqn:additive-noise-mechanism-ldp-measurement}.
\EndIf \label{line:8-end-add-noise}

\State The cloud estimator uses the $m$ measurement sets containing the protected measurements to perform the estimation process according to the following steps:
\State Compute the predicted state set {\color{blue}$ \mathcal{\hat{Z}}^{DP}_{k}= \zono{\hat{c}^{DP}_k, \hat{G}^{DP}_k}$} as follows:{\color{blue}
% \label{eqn:dp-time-update}
    % \mathcal{\hat{Z}}^{DP}_{k}=f(\mathcal{\Bar{Z}}^{DP}_{k-1})\oplus \mathcal{Z}_w \oplus \mathcal{\Bar{Z}}_{L,k},
\begin{align}
    \hat{c}^{DP}_k =&f({x_{k-1}^{*}})+\frac{\partial f_{k-1}}{\partial x}|_{x_{k-1}^{*}}\Big(\hat{c}^{DP}_{k-1} {-} x_{k-1}^{*}\Big) {+} c_{L,k},\label{eqn:dp-time-update-zonotope-center-non-linear}
\end{align}
\begin{align}
    \hat{G}^{DP}_k =&\bigg[\frac{\partial f_{k-1}}{\partial x}|_{x_{k-1}^{*}}\hat{G}^{DP}_{k-1}, G_{L,k}, G_w\bigg] ,\label{eqn:dp-time-update-zonotope-generator-non-linear}
\end{align}
where the center of the state, $x_{k-1}^{*}$, is used as a linearization point for the state function $f$ at time step $k-1\in \mathbb{Z}^+$. The infinite Taylor series is over-approximated by the first-order Taylor series and its Lagrange remainder $\mathcal{{Z}}_{L,k} = \zono{c_{L,k}, G_{L,k}}$.}\label{line:10-predicted-state-set} 
%in \eqref{eqn:dp-time-update}.
\State Compute the corrected state set $\mathcal{\Bar{Z}}^{DP}_{k}=\zono{\Bar{c}^{DP}_k, \Bar{G}^{DP}_k}$ in lines \ref{line:12} to \ref{line:17}.
%in \eqref{eqn:dp-estimation-with-zonotope-center-non-linear}, \eqref{eqn:dp-estimation-with-zonotope-generator-non-linear}.
\State\begin{align}
    \Acute{c}^{DP}_k =&  \hat{c}^{DP}_{k} + \sum_{i=1}^{m} \lambda^{(i)}_{k} \bigg( y^{(i)^{DP}}_{k} - h^{(i)}\big({x_{k}^{*}}\big)\nonumber\\ 
&-\frac{\partial h_{k}^{(i)}}{\partial x}|_{x_{k}^{*}}(\hat{c}^{DP}_{k} {-} x^{*}_{k}) {-} c_{L,k} 
% -c_{p} - c^{(i)}_{v} 
\bigg),\label{eqn:dp-estimation-with-zonotope-center-non-linear}
\end{align}
%$\Acute{c}^{DP}_k =  \hat{c}^{DP}_{k} + \sum_{i=1}^{m} \lambda^{(i)}_{k} \big ( y^{(i)^{DP}}_{k} - h^{(i)}({x_{k}^{*(i)}}) $\par$\quad\quad\;-\frac{\partial h_{k}^{(i)}}{\partial x}|_{x_{k}^{*(i)}}(\hat{c}_{k} {-} x^{*(i)}_{k}) {-} c^{(i)}_{L,k} \big)$, 


% \If{The model is Linear \eqref{eqn:system-model} }
% \State $\Acute{c}^{DP}_k =  \hat{c}^{DP}_{k} + \sum_{i=1}^{m} \lambda^{(i)}_{k} \big ( \hat{y}^{(i)^{DP}}_{k} - H^{(i)} \hat{c}^{DP}_{k} - c^{(i)}_{v}-c_{p} \big)$, 
% \State $\Acute{G}^{DP}_{k} =\bigg[(I- \sum_{i=1}^{m+1} \lambda^{(i)}_{k} H^{(i)})\hat{G}^{DP}_{k},$\par
% $\quad \quad \quad \; \; \lambda^{(1)}_{k} G^{(1)}_{v},\dots, \lambda^{(m)}_{k} G^{(m)}_{v}, \lambda^{(m+1)}_{k}{G}_{p}\bigg]$.
% \ElsIf{The model is non-linear \eqref{eqn:system-model-non-linear}}
\label{line:12}
\State  
\begin{align}
    \Acute{G}^{DP}_k =&\bigg[\bigg(I- \sum_{i=1}^{m} \lambda^{(i)}_{k} 
    \frac{\partial h_{k}^{(i)}}{\partial x}|_{x_{k}^{*}}
    \bigg) \hat{G}^{DP}_{k},\;-\lambda^{(1)}_{k} G_{L,k},\dots, \;\nonumber\\& -\lambda^{(m)}_{k} G_{L,k},-\lambda^{(1)}_{k}G_{p},\dots,-\lambda^{(m)}_{k}G_{p},\;\nonumber\\& -\lambda^{(1)}_{k}G^{(1)}_{v}, \dots, -\lambda^{(m)}_{k}G^{(m)}_{v}  \bigg].\label{eqn:dp-estimation-with-zonotope-generator-non-linear}
\end{align}
% where $G_{p}$ is the generator matrix, created using the range of the optimal noise $d$.
%$\Acute{G}^{DP}_k =\Big[\big(I- \sum_{i=1}^{m} \lambda^{(i)}_{k} \frac{\partial h_{k}^{(i)}}{\partial x}|_{x_{k}^{*(i)}} \big) \hat{G}^{DP}_{k},\;-\lambda^{(i)}_{k} G^{(i)}_{L,k}, $\par$\quad \quad \; \; -\lambda^{(i)}_{k}G_{p},\; -\lambda^{(1)}_{k}G^{(1)}_{v}, \dots, -\lambda^{(m)}_{k}G^{(m)}_{v}  \Big]$.
% \EndIf 
where the center of the state, $x_{k}^{*}$, is used as a linearization point at time step $k\in \mathbb{Z}^+$. The infinite Taylor series is over-approximated by the first-order Taylor series and its Lagrange remainder $\mathcal{{Z}}_{L,k} = \zono{c_{L,k}, G_{L,k}}$ to guarantee true state inclusion.
\State Compute the weights $\Bar{\Lambda}_k^*$
\begin{equation}\label{eqn:dp-optimal-lambda-weights}
\Bar{\Lambda}_k^* = \argminB_{{\lambda}_k}\lVert \Acute{G}^{DP}_k \rVert_{F}^{2},
\end{equation}
where $\Bar{\Lambda}_k^* = [ {\lambda}^{(1)}_{k},\dots,\; {\lambda}^{(m)}_{k}]$. \label{line:14-optimal-weights} 

% in \eqref{eqn:dp-optimal-lambda-weights}. 
% $= \argminB_{{\lambda}_k}\lVert \Acute{G}^{DP}_k \rVert_{F}^{2}$.
 
\State Reduce the order of $\Acute{G}^{DP}_k$ 
as in \cite{10.1007/978-3-540-31954-2_19}: $\Bar{G}^{DP}_{k} =\downarrow_q	\Acute{G}^{DP}_k$. 
\State $\Bar{c}^{DP}_k = \Acute{c}^{DP}_k$.
\State $\mathcal{\Bar{Z}}^{DP}_{k}= \zono{\Bar{c}^{DP}_k, \Bar{G}^{DP}_k}$. \label{line:17}
\State Update the time: $k=k+1$. \label{line18:time-step}
\EndWhile
\end{algorithmic}
\end{algorithm}

==> Sections/old-dp-prem.tex <==

Let $\mathcal{D}$ denote a space of datasets of interest, which are the global measurement signals $y$ released as a list of measurements vectors $\{y_k\}_{k\in\{1,\dots,\mathcal{T}\}}$, where $\mathcal{T}=\infty$ is also of interest and $y_k=\big[{y_k^{(1)}},\dots,{y_k^{(m)}}\big]^T$ \cite{9147726}.  
We aim to provide a certain level of privacy protection for an individual entity's measurement.
%; therefore, the state estimates should be insensitive to its contribution to the global measurement signals $y$.
Two global measurement signals $y$ and $\Acute{y}$ are called adjacent and can be denoted by Adj$(y,\Acute{y})$, if and only if they differ by the value of exactly one entity's measurement $y_k^{(i)}, \; i \in \{ 1,\dots,m\}$ \cite{degue2017differentially,9147726,6483414}. In other words, $y$ and $\Acute{y}$ are considered adjacent if there is any time step $k$ at which $y_k^{(i)}\neq\Acute{y}_k^{(i)}$. Since the privacy-preserving noise is added to the measurements themselves,
% and not to the queries applied to them,
then the allowed variation within Adj$(y,\Acute{y})$ is bounded by what is called sensitivity, which is defined formally as follows.

\begin{definition} [Sensitivity \cite{9147726,6483414}]
\label{def:sensitivity}
The allowed deviation for a single sensor's measurement between two adjacent global measurement signals $y$ and $\Acute{y}$, i.e., Adj$(y,\Acute{y})$, is bounded in the $L_2$ norm by $s$ and given by 
\begin{align}
\lVert y-\Acute{y}\rVert_2 \leq s,
\end{align}
where $s\geq0$.
\end{definition}
 % It deserves noting that $y$ and $\Acute{y}$ are considered different if there is any time step $k$ at which $y_k^{(i)}\neq\Acute{y}_k^{(i)}$.
Given a pair of adjacent global measurement signals, i.e., Adj$(y,\Acute{y})$, a differentially private mechanism aims to prevent an adversary from inferring knowledge about an individual entity's measurement by generating randomized outputs with close distributions for adjacent inputs.
{We use a pair of non-negative constants $(\epsilon,\delta)$ to quantify the privacy loss \cite{10.1007_11787006_1,degue2017differentially}. In particular, $e^{\epsilon}$ represents the ratio of probabilities to obtain the same state estimates with adjacent global measurement signals $y$ and $\Acute{y}$, and $\delta$ allows a small degree of violation when bounding the ratio of probabilities.}

\begin{definition} [Approximate Differential Privacy (ADP) \cite{10.1007_11787006_1,degue2017differentially}]
\label{def:approximate-dp} 
% Let the space of measurements $y$ denoted by $\mathcal{D}$. 
A randomized mechanism ${M}$, that maps the measurements' space $\mathcal{D}$ equipped with a sensitivity $s$ (Definition \ref{def:sensitivity}) to an anonymized measurements' space $\mathcal{O}$, is $(\epsilon,\delta)$-ADP if $\forall$ $\mathcal{H} \in \mathcal{O}$ and $\forall$ Adj$(y,\Acute{y}) \in \mathcal{D}$
\begin{align}\label{eqn:adp-formula}
	Pr\bigl[M(y)\in\mathcal{H}\bigl]\leq e^{\epsilon} Pr\bigl[M(\Acute{y})\in\mathcal{H}\bigl]+\delta, 
\end{align}
such that $\epsilon,\delta \geq 0$. If $\delta=0$, ${M}$ is said to be $\epsilon$-differentially private.
%\hfill $\square$
\end{definition}


\text{Differential Privacy models:}{\begin{itemize}
    \item {Central Differential Privacy (CDP).} 
    % The traditional model of differential privacy, in which a trusted data curator adds uncertainty (e.g., random noise) to the results of any processing on a centrally-held dataset to preserve the privacy of the participants in this dataset and prevent any untrusted party from inferring knowledge about an individual participant \cite{10.5555/3310435.3310586}.
    This traditional model of differential privacy involves a trusted data curator adding uncertainty, such as random noise, to the results of any processing on a centrally held dataset. This is done to safeguard the privacy of participants in the dataset and prevent any untrusted party from deducing information about individual participants \cite{10.5555/3310435.3310586}.
    \item {Local Differential Privacy (LDP).} 
    % In this model of differential privacy, the data of each Participant is locally perturbed, and the privacy-preserving process is transferred from the data curator to individual participants
    In this model of differential privacy, instead of centrally perturbing the data, each participant perturbs their own data locally before sharing it. This decentralized approach shifts the responsibility of privacy preservation from a central data curator to individual participants. Each participant adds noise to their own data before transmitting it to the data curator or any other party, ensuring that privacy is preserved at the local level \cite{Xiong2020}. 
\end{itemize}}

























%old Evaluation-two-examples

\section{Evaluation} \label{sec:eval}
% In this section, we evaluate the proposed $(\epsilon,\delta)$-ADP differentially private set-based estimator for the CDP and LDP setups. We present the experimental results for the Matlab R2023b implementation of our proposed $(\epsilon,\delta)$-ADP set-based estimator. For zonotope operations, we use the CORA toolbox.
This section evaluates the proposed $(\epsilon, \delta)$-ADP differentially private set-based estimator in both the CDP and LDP setups. Experimental results are presented based on the implementation in MATLAB R2023b, with zonotope operations performed using the CORA toolbox.


\subsection{The CDP Setup}\label{Evaluation-for-The-CDP-Setup}
% In this subsection, we evaluate the $(\epsilon,\delta)$-ADP differentially private set-based estimator within the context of the CDP setup using two localization examples.
% The first example is %Consider
% a network of $8$ sensory nodes tracking the location of an object in a circular motion within two-dimensional space with dimensions of $180\; \times 180\; m^2$ \cite{conf:disdiff}.
In this subsection, we evaluate the $(\epsilon, \delta)$-ADP differentially private set-based estimator within the context of the CDP setup through two localization examples. The first example involves a network of 8 sensory nodes tracking the location of an object moving in a circular motion within a two-dimensional space measuring $180\; \times 180\; m^2$ \cite{conf:disdiff}.
We aim to keep the sensory nodes' measurements private from the cloud estimator while estimating the location of the rotating object.
% The state of each node consists of two variables representing the position of the rotating object. 
The state of each node comprises two variables representing the position of the rotating object. 
The model of this system encompasses linear state and measurement functions, represented by the matrices $F$ and $H^{(i)}$, respectively, as follows:
% The state and measurement matrices are, respectively, as follows: 
\begin{equation*}
 F=\begin{bmatrix}
0.9920 & -0.1247 \\
0.1247 & 0.9920 
\end{bmatrix},\;
H^{(i)}=\begin{bmatrix}
1 &0 \\ 
\end{bmatrix}\; \mathrm{or}\;
\begin{bmatrix}
0 &1 
\end{bmatrix},
\end{equation*}
where the measurement matrix $H^{(i)}$ is selected based on the measurement sequence. The measurement and process noise zonotopes $\mathcal{Z}^{(i)}_{v}$ and $\mathcal{Z}_{w}$ are, respectively, set to: 
\begin{equation*}
    z^{(i)}_{v}=\Big\langle{\begin{bmatrix} 0 \end{bmatrix},\begin{bmatrix} 0.01\;\; 0.02 \end{bmatrix}} \Big\rangle
,\;
    z_{w}=\Bigg\langle{\begin{bmatrix} 0 \\0 \end{bmatrix},\begin{bmatrix} 0.50 & 0 \\0 & 0.50 \end{bmatrix}} \Bigg\rangle.
\end{equation*}
The $(\epsilon,\delta)$-ADP truncated optimal noise distribution (Definition \ref{def:optimal-noise}) is generated according to the noise model \eqref{eqn:noise-model} with $C=500$ in order to allow sudden jumps for the noise function $P(\phi_l)$. We set $d\in[-7,\;7]$, $\epsilon=0.3$, and $s=1$ and the parameters $A$, $B_j$, $F_j$, and $\delta$ are learned to optimize the loss function \eqref{eqn:optimization-function} using the SGD tool \cite{DBLP:journals/corr/abs-2107-12957}.

Figure \ref{fig:Object-tracking} represents a random snapshot for tracking the rotating object. We notice that the rotating object is enclosed by the estimated zonotope, which indicates that the state containment is still guaranteed, and the center of the estimated zonotope is very close to the rotating object, which is a good utility indicator. Supporting the above, Figure \ref{fig:estimated-location-error-with-epsilon} illustrates that the utility loss, represented by the standard deviation of the error in the estimated location of the rotating object, increases as the privacy budget $\epsilon$ decreases. It also indicates that as the $(\epsilon,\delta)$-ADP optimal noise range widens, there is a noticeable increase in both utility loss and average error in the estimated location of the rotating object.
%It also shows that utility losses and average errors in estimated locations of the rotating object increase with a wider $(\epsilon,\delta)$-ADP optimal noise range.
Hence, in industrial applications, for a certain privacy budget $\epsilon$, the selection of the optimal noise range $d$ should be guided by the acceptable error ranges.
% An industrial application should select the appropriate noise range based on the accepted error ranges.

For comparison, we consider the work in \cite{9147726}, where a differentially private interval estimator deploying truncated Laplace noise is presented. 
In particular, we compare the utility loss of $(\epsilon,\delta)$-ADP truncated optimal noise 
% (Definition \ref{def:optimal-noise})
and truncated Laplace noise \cite{9147726} at $\epsilon=0.3$. The results are shown in Figure \ref{fig:Estimation-error-vs-noise-acc-vs-optimal}. The truncated Laplace noise range, for a given $\epsilon,\delta$, and sensitivity $s$, is determined by 
\begin{equation}
a=\frac{s}{\epsilon}\ln{\Big(1+e^{\epsilon}\frac{1-e^{-\epsilon}}{2\delta}\Big)}.    
\end{equation}
At a certain $\delta$ value, we find that the truncated Laplace noise causes a higher utility loss than the $(\epsilon,\delta)$-ADP truncated optimal noise. Similarly, Figure \ref{fig:deltavs-noise-range} indicates that the truncated Laplace noise needed to achieve a certain $\delta$ is wider than the $(\epsilon,\delta)$-ADP truncated optimal noise needed to achieve the same $\delta$. Indeed, for a certain privacy budget $\epsilon$, learning the truncated optimal noise distribution $P(\phi_l)$ 
% (Definition \ref{def:optimal-noise})
using the SGD tool in \cite{DBLP:journals/corr/abs-2107-12957} allows our proposed $(\epsilon,\delta)$-ADP set-based estimator (Algorithm \ref{alg:adp-set-estimation-using-zonotope}) to minimize loss of privacy and utility simultaneously. 

%For LDP setup,
% The second example is the localization of a quad-copter that moves in arbitrary nonlinear motion within three-dimensional space with dimensions of $10\; \times \; 10 \; \times \; 10 \;m^3$ using a high rate of measurements provided by a set of $8$ anchor nodes distributed across the motion area. The state matrix is as follows: 
The second example involves the localization of a quad-copter navigating through arbitrary non-linear motion within three-dimensional space measuring $10\; \times\; 10\; \times\; 10\;m^3$. This localization is achieved using a high rate of measurements provided by a set of $8$ anchor nodes distributed across the motion area. The model of this system incorporates a linear state function represented by the matrix $F$, which is given by
\begin{equation*}
 F=\begin{bmatrix}
1 & 0 & 0\\
0 & 1 & 0\\
0 & 0  & 1
\end{bmatrix},\;
\end{equation*}
% The measurement matrix in this example is replaced by the nonlinear
Additionally, the measurement function $h^{(i)}(x_k)$ is defined as
\begin{equation*}
    h^{(i)}(x_k)=\lVert x_A^{(i)}-x_k\rVert\;_2, 
\end{equation*}
% function $h^{(i)}(x_k)=\lVert x_A^{(i)}-x_k\rVert\;_2 $, 
where $x_A^{(i)}$ represents the location of anchor node $i$ and $x_k$ is an estimate for the location of the quad-copter at time step $k$. 
The measurement and process noise zonotopes $\mathcal{Z}^{(i)}_{v}$ and $\mathcal{Z}_{w}$, respectively, are set to: 
\begin{equation*}
    z^{(i)}_{v}=\Big\langle{\begin{bmatrix} 0 \end{bmatrix},\begin{bmatrix} 0.01\;\; 0.02\;\; 0.01 \end{bmatrix}} \Big\rangle
,\end{equation*}
\begin{equation*}
    z_{w}=\Bigg\langle{\begin{bmatrix} 0 \\0\\0 \end{bmatrix},\begin{bmatrix} 0.50 & 0 & 0 \\ 0 & 0.50 & 0\\ 0 & 0 & 0.50 \end{bmatrix}} \Bigg\rangle.
\end{equation*}
The $(\epsilon,\delta)$-ADP truncated optimal noise distribution
% (Definition \ref{def:optimal-noise})
is regenerated using the same parameters as in the first example except for $d\in[-1,\;1]$. Again, we compare the utility loss, represented by the second norm of the error in the estimated location of the quad-copter, associated with the $(\epsilon,\delta)$-ADP truncated optimal noise
% (Definition \ref{def:optimal-noise})
and the truncated Laplace noise \cite{9147726} at $\epsilon=0.3$. The results presented in Figure \ref{fig:Estimation-error-vs-noise-acc-vs-optimal-quad-copter-CDP} demonstrate that the utility loss incurred when employing the $(\epsilon,\delta)$-ADP truncated optimal noise is lower than that observed with the truncated Laplace noise at certain privacy level.

%results in less error in the estimated location of the quad-copter than using the truncated Laplace noise distribution. 

From the comparative results in the two preceding examples, we can notice that the proposed $(\epsilon,\delta)$-ADP set-based estimator causes less utility loss than the differentially private interval estimator, proposed in \cite{9147726}, 
in the context of the CDP setup.


 



\begin{figure}[h]
\graphicspath{ {./Figures/} }
    \centerline{
\includegraphics
[scale=0.42]{Figures/Object-tracking-180x180}}
    \caption{Tracking an object in circular motion,  {\img{Figures/box}}: rotating object, {\img{Figures/triangle}}
    : sensory nodes, {\color{red}+} : center of the estimated zonotope.}
    \label{fig:Object-tracking}
\end{figure}

\begin{table*}[htbp]\centering 
%\ra{1.3}
\begin{small}
\begin{tabular}{@{}lrrrrrrrrrrrr@{}}\toprule
{$\epsilon$\;/\;Noise Range $d(m)$} & {3} & {5} & {7} & {9} & {11} & {13} & {15} \\ \midrule
{0.1} & 0.1502\ & 0.0811\ & 0.0518\ & 0.0360\ & 0.0262\ & 0.0197\ & 0.0151\ \\ 
{0.3} & 0.1198\ & 0.0503\ & 0.0244\ & 0.0126\ & 0.0067\ &0.0036\ & 0.0020\ \\ 
{0.5} & 0.0931\ & 0.0290\ & 0.0101\ & 0.0036\ & 0.0013\ & 0.0005\ & 0.0002\ \\ %\hdashline
{0.7} & 0.0707\ & 0.0158\ & 0.0038\ & 0.0009\ & 0.0002\ & $5.64e^{-5}$\ & $1.39e^{-5}$\ \\ %\hdashline
\bottomrule
\end{tabular}
\end{small}
\caption{Optimal $\delta$ values corresponding to different ranges $d(m)$ of $(\epsilon,\delta)$-ADP optimal noise at $\epsilon={0.1,0.3,0.5,0.7}$.}
\end{table*}



\subsection{The LDP Setup}\label{Evaluation-for-The-LDP-Setup}
In this subsection, we evaluate the proposed $(\epsilon,\delta)$-ADP differentially private set-based estimator within the context of the LDP setup. We conduct the evaluation using the localization of a quad-copter navigating arbitrary non-linear motion within three-dimensional space, with dimensions of $10\; \times \; 10 \; \times \; 10 \;m^3$. The quad-copter's localization is achieved through a high rate of measurements provided by a set of $8$ anchor nodes distributed across the motion area. It deserves mentioning that the sensor manager is not present to aggregate the measurements of the sensors since it is treated as an untrusted entity in the LDP setup. Instead, each sensor locally perturbs its own measurement with the privacy-preserving noise.

As in the CDP setup of this example, the $(\epsilon,\delta)$-ADP truncated optimal noise distribution 
% (Definition \ref{def:optimal-noise})
is regenerated for the LDP setup. In the context of the LDP setup, we again compare the utility loss of $(\epsilon,\delta)$-ADP truncated optimal noise 
% (Definition \ref{def:optimal-noise}) 
and truncated Laplace noise \cite{9147726} at $\epsilon=0.3$. 
% The results are shown in Figure \ref{fig:Estimation-error-vs-noise-acc-vs-optimal-quad-copter-LDP}.
The comparative results in Figure \ref{fig:Estimation-error-vs-noise-acc-vs-optimal-quad-copter-LDP} demonstrate that in the proposed $(\epsilon,\delta)$-ADP set-based estimator, utilizing $(\epsilon,\delta)$-ADP truncated optimal noise leads to less utility loss compared to employing truncated Laplace noise \cite{9147726} in the context of the LDP setup.
% From the comparative results in Figure \ref{fig:Estimation-error-vs-noise-acc-vs-optimal-quad-copter-LDP}, we can notice that the proposed $(\epsilon,\delta)$-ADP set-based estimator, utilizing the $(\epsilon,\delta)$-ADP truncated optimal noise, also outperforms the differentially private interval estimator, employing truncated Laplace noise \cite{9147726}, in the context of LDP setup by achieving less utility loss.
%resulting in less utility loss using the LDP setup.



% Additionally, our proposed $(\epsilon,\delta)$-ADP set-based estimator (Algorithm \ref{alg:adp-set-estimation-using-zonotope}) leverages zonotopes for set representation. The zonotopes are less conservative set representation that allow efficient computation of linear maps and Minkowski sum, which are essential operations at the set-based estimation process. 
% This in turn gives the proposed $(\epsilon,\delta)$-ADP set-based estimator a computational advantage.
Furthermore, our proposed $(\epsilon,\delta)$-ADP set-based estimator (Algorithm \ref{alg:adp-set-estimation-using-zonotope}) utilizes zonotopes for set representation. Zonotopes offer a less conservative set representation that enables efficient computation of linear maps and Minkowski sums, both essential operations in the set-based estimation process.
Consequently, this confers a computational advantage to the proposed $(\epsilon,\delta)$-ADP set-based estimator.

\begin{figure}[t]
\graphicspath{ {./Figures/} }
    \centerline{
\includegraphics
[scale=0.56]{Figures/Estimation-error-vs-noise-range2}}
    \caption{Effect of $(\epsilon,\delta)$-ADP optimal noise range on the average error in the estimated location of the rotating object. }
    \label{fig:estimated-location-error-with-epsilon}
\end{figure}


\begin{figure}[t]
\graphicspath{ {./Figures/} }
\centerline{\includegraphics[scale=0.56]{Estimation-error-vs-noise-acc-vs-optimal2}}
\caption{
% Comparing the effect of $(\epsilon,\delta)$-ADP truncated optimal noise and truncated Laplace noise on the error at the estimated location of the rotating object at $\epsilon=0.3$.
Comparison of the impact of $(\epsilon, \delta)$-ADP truncated optimal noise and truncated Laplace noise on the error in the estimated location of the rotating object, with $\epsilon = 0.3$.}
\label{fig:Estimation-error-vs-noise-acc-vs-optimal}
\end{figure}
